Adaptive Sampling for Convex Regression

In this paper, we introduce the first principled adaptive-sampling procedure for learning a convex function in the $L_\infty$ norm, a problem that arises often in the behavioral and social sciences. We present a function-specific measure of complexity and use it to prove that, for each convex function $f_{\star}$, our algorithm nearly attains the information-theoretically optimal, function-specific error rate. We also corroborate our theoretical contributions with numerical experiments, finding that our method substantially outperforms passive, uniform sampling for favorable synthetic and data-derived functions in low-noise settings with large sampling budgets. Our results also suggest an idealized "oracle strategy", which we use to gauge the potential advance of any adaptive-sampling strategy over passive sampling, for any given convex function.

==> approx_complex.tex <==
%!TEX root = manuscript.tex


\subsection{Sample Complexity of Approximating a Convex Function}\label{sec:lowerbounds}

We first consider the passive uniform sampling scheme where $x_i = \frac{i}{n-1}$ for $i=1,\dots,n-1$ for some value of $n$. If $x_* := \arg\inf\left\{\omega(f,x,\epsilon) :x \in [\tleft(f,\epsilon),1 - \tright(f,\epsilon)]  \right\} $ and no $x_i$ was contained in $I_* := [x_*-\omega(f,x_*,\epsilon),x_*+\omega(f,x_*,\epsilon)]$, then it would be impossible to disambiguate between $f(x)$ and the function $\tilde{f}_{I^*} := f(x) + \I(x \in I^*) \cdot
\left(\Sec[f,I^*](x) - f(x)\right)$, the function obtained by replacing $f$ with its secant approximation on $I^*$, with an approximation error less than $\epsilon$.
This implies that any $(\epsilon,\delta)$-correct uniform sampling procedure requires $n \gtrsim \sup_{x \in [\tleft(f,\epsilon),1 - \tright(f,\epsilon)]} \omega(f,x,\epsilon)^{-1}$ measurements to ensure that $1/(n-1)$ is smaller than $|I_*|=\inf_{x \in [0,1]} 2\omega(f,x,\epsilon)$.


By the same token, if any (even adaptive) algorithm does not measure $f$ on an interval $I$ for which $\Delta(f,I) \ge \epsilon$, then $f$ cannot distinguish between $f$ and the alternative function $\tilde{f}_I := f(x) + \I(x \in I) ( \Sec[f,I](x) - f(x))$. Thus, a key step to showing that $\Lambda(f,\epsilon)$ effectively lower bounds the number of evaluations is to show that it roughly lower bounds the number of intervals $I$ for which $\Delta(f,I) \ge \epsilon$.
The following packing lemma is proved in Section~\ref{sec:packing_proof}.

%Now let us consider arbitrary sampling patterns of $n$ points in $[0,1]$ to obtain a lower bound on any algorithm that chooses locations to sample sequentially and adaptively.
\begin{lemma}[Packing] \label{lem:packing}\vspace{-1pt}
Let $f:[0,1] \rightarrow \R$ be a convex function, $\epsilon>0$, and define
\begin{eqnarray}
\underline{N}(f,\epsilon) = \frac{\Lambda(f,\epsilon)}{4(1+\log(\omega_{\max}(f,\epsilon)/\omega_{\min}(f,\epsilon)))} - 3
\end{eqnarray}
where $\omega_{\max}(f,\epsilon) = \max_{x \in [\tleft(f,\epsilon),1-\tright(f,\epsilon)]}\omega(f,x,\epsilon)$ and $\omega_{\min}$ is defined analogously. Then, for any $n \leq \underline{N}(f,\epsilon)$ there exists $\{z_i\}_{i=1}^n \subset [0,1]$ such that the intervals $I^{\epsilon}_i := [z_i - \omega(z_i,f,\epsilon),z_i + \omega(z_i,f,\epsilon)]$ have disjoint interiors, are contained in $[2\tleft(f,\epsilon),1-2\tright(f,\epsilon)]$  and satisfy $\sup_{x \in I^{\epsilon}_i} \Sec[f,I^{\epsilon}_i](x) - f(x) \geq \Delta(f,I_i^{\epsilon}) > \epsilon$ for all $i$.
\end{lemma}
Thus, if we define the local class of alternatives functions (all of which are also convex)
\begin{align}\label{Local_Alternatives_Eq}
\mathcal{G}_{f,\epsilon} := \Big\{ f(x) + \sum_{i=1}^n \beta_i \I\{ x \in I^{\epsilon}_i \}(\Sec[f,I^{\epsilon}_i](x)-f(x)) : \beta \in \{0,1\}^{n} \Big\},
\end{align}
then $f \in \mathcal{G}_{f,\epsilon}$ and for any $\{x_i\}_{i=1}^{n-1} \subset [0,1]$ there exists a convex function $g \in \mathcal{G}_{f,\epsilon}$ such that $f(x_i) = g(x_i)$ for all $i$ and $\sup_{x \in [0,1]} g(x) - f(x) > \epsilon$. Hence, if a sample is not placed in each interval $I_i^{\epsilon}$, one cannot disambiguate between the true function $f$ and the $g \in \mathcal{G}_{f,\epsilon}$ that differs by $f$ only over the interval $I_i^{\epsilon}$. Inflating $\epsilon$ by a factor of $2$ a we see that if $\Alg$ cannot distinguish between $f$ and $g \in \calG_{f,2\epsilon }$, then $f$ will incur an error  $> \epsilon$ on one of the two instances. Thus,

\begin{theorem}[Active Lower Bound - Noiseless] \label{thm:lowerbound_noiseless}
Fix some convex function $f$ and $\epsilon >0$.
Let $\underline{N}(f,\epsilon)$ and $\mathcal{G}_{f,2\epsilon}$ be defined as in Lemma~\ref{lem:packing} and Equation~\eqref{Local_Alternatives_Eq}.
If $\Alg$ is $(\epsilon,\delta)$-correct over the class $\calG_{f,2\epsilon}$, then
% \begin{eqnarray}
$\E_{f,\Alg}[T]  \ge (1-2\delta)\underline{N}(f,2\epsilon)$.
% \end{eqnarray}
\end{theorem}
The above theorem, whose proof is found in Section~\ref{sec:proof_lowerbound_noiseless}, demonstrates a lower bound on the true number of samples collected when approximating $f$, provided that $\Alg$ is uniformly correct over the class of instances $\calG_{f,2\epsilon}$. While the above lower bound holds a fortiori for the class of all convex functions, we emphasize that it applies \emph{even} when we consider these local alternatives.

By inspecting the proof of the packing, we see that we can \emph{cover} the interval $[0,1]$ with $\underline{N}(f,\epsilon) + 3$ intervals $I$ such that $\Delta(f,I) = \epsilon$. By our main lemma, this implies that obtaining noiseless measurements of $f$ on the endpoints and midpoints of these intervals is sufficient to certify that the estimator $\widehat{f}$ obtained via the secant approximation to $f$ on each interval, using the measurements, satisfies $\|\widehat{f} - f\|_{\infty} \le 2\epsilon$. We therefore refer to the consturction in our packing as the \emph{oracle strategy}, since it constitutes the best possible allocation of samples for identifying $f$ up to a constant rescaling of $\epsilon$ (adressed below), and a small additive constant.
Suprisingly, a close approximation to this oracle strategy can be attained by efficient sampling procedure, detailed in Section~\ref{sec:noiseless_alg}. We state its guarantee as follows:
\begin{theorem}\label{thm:upperbound_samples_noiseless}
Let $f:[0,1] \rightarrow \R$ be convex, let $\Alg$ denote the algorithm of Section~\ref{sec:noiseless_alg}, and fix $\epsilon > 0$. Then once $\Alg$ evaluates $f$ at $n = \overline{N}(f,\epsilon) := \ceil{ 12 \Lambda(f,\epsilon/2) + 9}$ locations, $\Alg$ can certify that the convex function $\widehat{f}_n$ defined in Section~\ref{sec:noiseless_alg} satisfies $\|f-\widehat{f}_n\|_{\infty} \le \epsilon$.
\end{theorem}
In the above theorem, $\Alg$ is able to certify $\|f - \widehat{f}_n\|_{\infty} \le \epsilon$ by measuring $f$ on the endpoints $\xl,\xr$ and midpoints $\xm$ of a family $\calI$ of adaptively chosen intervals , such $\bigcup_{I \in \calI} I =[0,1]$, and $\Delta(f,I) \le \epsilon/2$ for all $I \in \calI$.
With this information, $\Alg$ can construct a secant approximation to $f$ on each interval which then satisfies $\sup|\Sec[f,x] - f(x)| \le 2 \cdot \epsilon/2 = \epsilon$ by Lemma~\ref{lem:mainLemmaSimple}.
The key challenge is designing the algorithm to only require $\lesssim \Lambda(f,\epsilon/2)$ of these intervals.



%In the Ap
%Consequently, for some $g \in \mathcal{G}_{f,\epsilon}$ let $\E_{g,\Alg}[T]$ be the expected number of noiseless observations made of $g$ taken before $\Alg$ outputs some %$\widehat{f}$ that satisfies $||g - \widehat{f}||_\infty < \epsilon$ with probability at least $1-\delta$.
%Then
%\begin{eqnarray}\label{SecondLB}
%\max_{g \in \mathcal{G}_{f,\epsilon}}
%\end{eqnarray}
%an $\max_{g \in \mathcal{G}_{f,\epsilon}} M(g,\epsilon) \leq {\color{red}2} M(f,\epsilon)$.
%\end{theorem}
% \begin{remark}
% The alternative functions in $\calG_{f,2\epsilon}$ are quite benign.
% For example, Proposition~\ref{LambdaScaleProp} shows that for any $c \le 1$, $\Lambda(g,c\epsilon) \le \frac{1}{c}\Lambda(f,\epsilon)$, which implies that the algorithm of Theorem~\ref{thm:upperbound_samples_noiseless} can learn any $g \in \calG_{f,2\epsilon}$ using at most $O(\Lambda(f,2\epsilon))$ samples. Moreover, if $f$ is either  $L$-Lipschitz, bounded as $a \le f \le b$, or monotone, then $g$ will be, respectively, $L$-Lipschitz, bounded as $a \le g \le b$, and monotone as well.
% \end{remark}

\subsection{Comparing the upper and lower bound}
The upper bound of Theorem~\ref{thm:upperbound_samples_noiseless} and lower bound of Theorem~\ref{thm:lowerbound_noiseless}, nearly match, with two exceptions:
The first is that the upper bound is in terms of $\Lambda(f,\epsilon/2)$, whereas the lower bound is in terms of $\Lambda(f,2\epsilon)$.
The two quantities can be related by the following proposition, proved in Appendix~\ref{Appendix:Technical}.
\begin{proposition}\label{LambdaScaleProp} For any $0 < c \le 1$, $\epsilon > 0 $ and any convex $f$, $\omega(f,x,\epsilon) \geq \omega(f,x,c \epsilon) \geq c \omega(f,x,\epsilon)$ for all $x \in [\tleft(f,\epsilon),1-\tright(f,\epsilon)]$.
Moreover,
\begin{eqnarray*}
 \Lambda(f,\epsilon) + \log\frac{\tleft(f,\epsilon)\tright(f,\epsilon)}{\tleft(f,c\epsilon)\tright(f,c\epsilon)} \le \Lambda(f,c\epsilon) \le \frac{1}{c}\left\{\Lambda(f,\epsilon) + \log\frac{\tleft(f,\epsilon)\tright(f,\epsilon)}{\tleft(f,c\epsilon)\tright(f,c\epsilon)} \right\}.
\end{eqnarray*}
\end{proposition}\vspace{-2pt}
Hence, ignoring the contributions of the endpoints $\tleft$ and $\tright$, rescaling $\epsilon$ by a multiplicative constant $c$ changes $\Lambda(f,\epsilon)$ by at most $c$.

The second gap in the upper and lower bounds comes from the fact that $\underline{N}(f,\epsilon)$ requires dividing through by $\log(\omega_{\max}/\omega_{\min})$.
This is not simply an artificat of the proof.
For example, for any $k$-piecewise linear function, there exists a set of $k$ intervals $\calI = \{I_i\}_{1 \le i \le k}$ such that $f$ is linear on each interval; measuring $f$ at $\{\xl,\xr,\xm\}_{I \in \calI}$ would be enough to estimate $f$ with zero-error.
Hence, we must have $\underline{N}(f,\epsilon) \lesssim k$.
On the other hand, $\Lambda(f,\epsilon) \approx k \log(1/\epsilon)$, and indeed one can show that for a $k$-piecewise linear function, $\log(\omega_{\max}/\omega_{\min}) \approx \log(1/\epsilon)$, yielding the necessary cancelation.
As with the term $\log\frac{\tleft(f,\epsilon)\tright(f,\epsilon)}{\tleft(f,c\epsilon)\tright(f,c\epsilon)}$, $\log(\omega_{\max}/\omega_{\min})$ grows like at most $\log(1/\epsilon)$ for most reasonable functions, and can be bounded by $\log(\max_{x \in [0,1]}f''(x)/\min_{x \in [0,1]} f''(x))$ for twice-differentiable functions $f$.
Overall, we conjecture that the true sample complexity lies closer to $\underline{N}(f,\epsilon)$, because in the noiseless setting, one can approximate left- and right-derivatives of $f$ to arbitrary accuracy using just two-points. This makes it possible to learn a 2-piecewise linear function with a constant number of function evaluations, rather than the $O(\log(1/\epsilon))$ implied by $\Lambda(f,\epsilon)$.

% To study the potential gains of active sampling, we consider two particular classes of functions.
% If $f$ is linear on $k$ disjoint intervals of $[0,1]$, as discussed above, then  $\Lambda(f,\epsilon) \approx k \log(1/\epsilon)$ while uniform passive sampling would have to wait to get a sample in the local neighborhood of each kink, requiring a sample complexity of $k /\epsilon$, an exponentially large gap.
% On the other hand, if $||f'''||_\infty < 0$ then $\omega(f,x,\epsilon) \approx \sqrt{2\epsilon/f''(x)}$ which implies that $\Lambda(f,\epsilon) \approx \epsilon^{-1/2} \int_0^1 \sqrt{f''(x)} dx$ whereas the granularity of uniform passive sampling would be dictated by the largest-curvature resulting in a sample complexity of $\epsilon^{-1/2} \max_{x \in[0,1]} \sqrt{f''(x)}$.


%In the next section, we propose an algorithm whose sample complexity we prove nearly matches this lower bound.
%In particular, we will show that any convex function $g$ with $\Lambda(g,\epsilon) \leq \Lambda(f,\epsilon)$ can be learned with just roughly $\Lambda(f,\epsilon)$ samples, implying that this is a fundamental quantity describing the sample complexity of learning a convex function using active sampling.

% As a sanity check, we see that $\omega(f,x,\epsilon)$ is non-increasing in $\epsilon$, and is equal to $1$ for all $x \in [0,1]$ when $f$ is affine. Moreover, as we show in Lemma~\ref{SecantProperties}, $\omega(f,x,\epsilon) > 0$ for all $x \in [0,1]$ and all $\epsilon >0$. Thus sample complexity results will be stated in terms of the average of the $1/\omega$, given by the integral $\int \omega(f,u,\epsilon)^{-1}du$.
% \maxs{Kevin Give Intuition}

\subsection{Recursive Secant Approximation Algorithm}\label{sec:noiseless_alg}
We now describe the algorithm that achieves the claimed sample complexity of Theorem~\ref{thm:upperbound_samples_noiseless}. Consider a binary tree $\Tcal$ whose nodes represent intervals on $[0,1]$ such that the root is $[0,1]$, and each internal node representing $[a,b]$ has children $[a,(a+b)/2]$ and $[(a+b)/2,b]$.
If the leaves of $\Tcal$ are denoted as $\Lcal(\Tcal)$ then we conclude that the intersection of any two leaves $I,I' \in \Lcal(\Tcal)$ is at most a point $|I \cap I'| = 0$, and that the leaves cover the full interval $\bigcup_{I \in \Lcal(\Tcal)} I = [0,1]$.
For a given tree $\Tcal$ and function $f$ define
$\Sec[f,\Tcal](x)$ as $\Sec[f,I](x)$ for the $I \in \Lcal(\Tcal)$ such that $x\in I$ (breaking ties arbitrarily).
% \begin{align}\label{eqn:noiseless_fhat}
% \Sec[f,\Tcal](x) =  \I\{ x \in \cup_{I \in \Lcal(\Tcal)} \partial I \} \ f(x) +   \sum_{I \in \Lcal(\Tcal)} \I\{ x \in \text{\sf int}(I) \} \ \Sec[f,I](x)
% \end{align}
% where for interval $[a,b]$ we define the boundary $\partial [a,b] = \{a, b\}$ and interior $\text{\sf int}([a,b]) = (a,b)$ so that $\partial [a,b] \cap \text{\sf int}([a,b]) = \emptyset$ and $\partial [a,b] \cup \text{\sf int}([a,b]) = [a,b]$.
Note that $\Sec[f,\Tcal](x)$ evaluates $f$ only at $|\Lcal(\Tcal)|+1$ locations. Moreover, we have that $\sup_{x \in [0,1]} | \Sec[f,\Tcal](x) - f(x)| \leq \max_{I \in \Lcal(\Tcal)} 2 \Delta(f,I)$ and given a tree $\Tcal$, one can compute $\Delta(f,I)$ for each $I \in \Lcal(\Tcal)$ using just $|\Lcal(\Tcal)|$ additional samples, which could then be reused if the leaves produced children.

Our algorithm starts with a tree $\Tcal$ of depth 2 such that $\Lcal(\Tcal) = \{ [0,1/2],[1/2,1] \}$ and at each time step, two children are appended to the leaf $\arg\max_{I \in \Lcal(\Tcal)} \Delta(f,I)$.
This process continues until the first time in which $\max_{I \in \Lcal(\Tcal)} \Delta(f,I) \leq \epsilon/2$.
Then it is easy to see that in the resulting tree, for each $I \in \Lcal(\Tcal)$ we have $\Delta(\parent(I)) > \epsilon/2$ and $\Delta(f,I) \leq \epsilon/2$.
Let $\Tcal'$ be the largest tree such that $\Delta(f,I) > \epsilon/2$ for all $I \in \Lcal(\Tcal')$.
If each leaf of $\Tcal'$ has two children then the resulting tree's leaves will each have $\Delta(f,I)\leq \epsilon/2$, and because $\Tcal'$ was the largest tree, we have $|\Lcal(\Tcal)| \leq 2|\Lcal(\Tcal')|$.
% $\sup_{x \in [0,1]} | \widehat{f}(x) - f(x)| \leq \epsilon$.
% , so the tree with the minimum number of leaves has no more than twice the number of leaves necessary to guarantee that each leaf in the tree has $\Delta(f,I) \leq \epsilon/2$.
% And if the resulting tree has $|\Lcal(\Tcal)|$ total leaves, the total number of evaluations of $f$, including those used to calculated $\Delta(f,I)$ for each $I \in \Lcal(\Tcal)$, is bounded by $2|\Lcal(\Tcal)| + 1$.
The next lemma, proved in Section~\ref{MidIntervalModulus}, will be instrumental in relating the cardinality of this $\epsilon/2$-suboptimal ``largest tree'' to a digestable quantity that depends only on $f$.
\begin{lemma}\label{MidIntervalModulus} Let $[a,b] \subset [0,1]$, and suppose that $\Delta(f, [a,b]) \ge \epsilon$. Then for any $\alpha \in (0,1)$,
% \begin{eqnarray}
$\int_{a}^b \omega(f,x,\epsilon(1 - \alpha))^{-1} dx\ge \frac{2\alpha}{1+\alpha}$.
% \end{eqnarray}
\end{lemma}


Recall the definition of $\Tcal'$ from above, where each $I \in \Lcal(\Tcal')$ satisfies $\Delta(f,I) > \epsilon/2$.
By definition, $\tleft(f,\epsilon/2) := \inf \left\{t \le 1/2: \Delta\left(f,[0,2t]\right) \ge \epsilon/2\right\}$ which implies that there is an $I_{left} \in \Lcal(\Tcal')$ such that $[0,2\tleft(f,\epsilon/2)] \subseteq I_{left}$, define $I_{right}$ analogously.
We can bound the number of leaves:
\begin{align*}
|\Lcal(\Tcal')| &=  2 + \sum_{I \in \Lcal(\Tcal') \setminus \{I_{left},I_{right}\}} 1
\overset{(i)}{\leq} 2 + \sum_{I \in \Lcal(\Tcal') \setminus \{I_{left},I_{right}\}} \frac{3}{2} \int_{x \in I} \omega(f,x,\epsilon/4 )^{-1} dx \\
&\overset{(ii)}{\leq} 2+ \frac{3}{2} \int_{2\tleft(f,\epsilon/2)}^{1-2\tright(f,\epsilon/2)} \omega(f,x,\epsilon/4 )^{-1} dx
\overset{(iii)}{\leq} 2+ 3 \int_{\tleft(f,\epsilon/2)}^{1-\tright(f,\epsilon/2)} \omega(f,x,\epsilon/2 )^{-1} dx\\
&= 2 + 3 \Lambda(f,\epsilon/2)
\end{align*}
where $(i)$ follows from Lemma~\ref{MidIntervalModulus} with $\alpha=1/2$ applied to each $I$ in the sum, $(ii)$ follows from the the fact that $[0,2\tleft(f,\epsilon/2)] \subseteq I_{left}$ and $[1-2\tright(f,\epsilon/2),1] \subseteq I_{right}$, and $(iii)$ follows from $\omega(f,x, \epsilon/4 ) \geq \frac{1}{2} \omega(f,x,\epsilon/2)$ for $x \in [\tleft(f,\epsilon/2),1-\tright(f,\epsilon/2)]$ by Proposition~\ref{LambdaScaleProp} and that we trivially have $[2\tleft(f,\epsilon/2),1-2\tright(f,\epsilon/2)] \subseteq [\tleft(f,\epsilon/2),1-\tright(f,\epsilon/2)]$.


By a calculation above, we concluded that a tree $\Tcal$ could be constructed (including validating that $\Delta(f,I) \leq \epsilon/2$ on the leaves) with just $2|\Lcal(\Tcal)|+1$ evaluations of $f$.
Since $|\Lcal(\Tcal)| \leq 2|\Lcal(\Tcal')|$, we conclude that $\Tcal$ is constructed after evaluating $f$ at most $9 + 12 \Lambda(f,\epsilon/2)$ times, obtaining the claimed result of Theorem~\ref{thm:upperbound_samples_noiseless}.


==> implementation.tex <==
%!TEX root = manuscript.tex
\section{Implementation of Numerical Experiments\label{implemtation}}

Let dyadic sampling on an interval $[a,b]$ be defined as the sequence $a+(b-a)\vec{s}$.
We consider three methods: 1) \texttt{passive-dyadic}: dyadic sampling on $[0,1]$, 2) \texttt{active}: Algorithm~\ref{Algorithm}, and 3) \texttt{active-dyadic}: on odd times sample according to Algorithm~\ref{Algorithm} and on even times pick the interval in $\Lcal(\Tcal)$ that has been sampled the fewest times on even times and sample at the next location in the dyadic sequence on that interval.   
Regardless of the method, to compute an estimator we use all the data collected from the method to compute the least squares estimator subject to the function being convex\footnote{For a finite number of observations, convex regression is a quadratic program \cite{boyd2004convex}.}\footnote{That is, the \texttt{active} estimator is \emph{not} a collection of secant approximations.}. 

We begin by confirming theoretical predictions. The empirical results are presented in Figure~\ref{fig:simulated_matrix} for $\sigma = .01$.
The dotted and solid lines represent the $L_\infty$ error on $[0,1]$ and $[0.1,0.9]$, respectively. 
%When $f(x)=1-x$ we should expect the \texttt{active} algorithm to never split, sample just at $\{0,1/2,1\}$, and to perform very similarly to \texttt{passive-dyadic}.


==> lambda_facts.tex <==
%!TEX root = manuscript.tex

\section{Discussion on $\Lambda(f,\alpha \epsilon)$ for $\alpha >0$} \label{sec:constant_relationship}


Let $f : \R \rightarrow \R$ be a convex function. 
If we ignore the boundary of $[0,1]$ in the defintion of $\omega(f,x,\epsilon)$, then $\omega(f,x,\epsilon)=t  \iff g(t) := \frac{f(x+t)+f(x-t)}{2}-f(x) = \Sec[f,[x-t,x+t]](x) - f(x) = \epsilon$. 
By convexity, we have $g( \lambda t ) = g( \lambda t + (1-\lambda) 0 ) \leq \lambda g(t) + (1-\lambda) g(0) = \lambda g(t)$ for any $\lambda \in [0,1]$.
As a consequence, 
\begin{align*}
\omega(f,x, \lambda g(t)) \geq \omega(f,x, g(\lambda t)) = \lambda t = \lambda \omega(f,x, g(t))
\end{align*}
which implies $\omega(f,x,\lambda \epsilon) \geq \lambda \omega(f,x, \epsilon)$ for any $\lambda \in [0,1]$, or $c \omega(f,x,\epsilon /c) \geq \omega(f,x,\epsilon)$ for any $c \geq 1$.

On the other hand, suppose $||f'''||_\infty < \infty$. 
Note that $g(0)=g'(0)=0$, and $g''(0) = f''(x) \geq 0$ because $f$ is convex.
This implies 
$g(t) =\frac{1}{2} g''(0) t^2 + \frac{1}{6} g'''(0) t^3 + \dots \overset{t \rightarrow 0}{=} \frac{1}{2} f''(x) t^2$ so that 
\begin{align*}
\omega(f,x,\alpha \epsilon) \overset{\epsilon \rightarrow 0}{=} \sqrt{ \frac{2 \alpha \epsilon}{f''(x)} } \overset{\epsilon \rightarrow 0}{=} \sqrt{\alpha} \ \omega(f,x, \epsilon) \qquad \alpha > 0.
\end{align*}

Of course, both of the above arguments ignored the endpoints in the definition of $\omega(f,x,\epsilon)$.
If $t_{L} = \min\{x : x \geq \omega(f,x,\epsilon)\}$ and $t_{R} = \max\{x : x \leq \omega(f,x,\epsilon)\}$ then the end points can be ignored on $[t_L, t_R] \subseteq [0,1]$. 
As $\epsilon \rightarrow 0$ we have $t_L \rightarrow 0$ and $t_R \rightarrow 1$ for any continuous, convex, bounded function $f$. 
Thus, as $\epsilon \rightarrow 0$ we argue that $\Lambda(f, \Theta(\alpha)) = \Theta(\Lambda(f,\epsilon))$.


==> lambda_facts_proof.tex <==
%!TEX root = manuscript.tex
\section{Technical Properties of}



\iffalse
\subsection{Further stuff?}




\begin{proposition}[Restatement and Extension of Proposition~\ref{LambdaScaleProp}]\label{GeneralLambdaScaleProp}
For all $\lambda \ge 1$
\begin{eqnarray}
\Lambda(f, \epsilon) \in [1,\lambda]\left\{\Lambda(f,\lambda\epsilon) + \log \frac{\tright(f,\lambda\epsilon)\tleft(f,\lambda\epsilon)}{\tright(f,\epsilon)\tleft(f,\epsilon)}) \right\}
\end{eqnarray}
Moreover,
\begin{eqnarray}
\log(\frac{\omega_{\max}}{\omega_{\min}}) \le \log (\|f\|_{\infty}/\epsilon) + \log(1/\tleft(f,\epsilon)) + \log(1/\tright(f,\epsilon))
\end{eqnarray}
and thus,
\begin{eqnarray}
\underline{N}(f,\epsilon) \gtrsim \frac{\Lambda(f,\epsilon)}{\log (\|f\|_{\infty}/\epsilon) + \log(1/\tleft(f,\epsilon)) + \log(1/\tright(f,\epsilon))}
\end{eqnarray}
\end{proposition}


\subsection{Preliminaries}
% In this section, we establish many useful regularity results about the $\tleft,\tright$ and $\omega$. We let $\overline{I}(f,\epsilon) = [\tleft(f,\epsilon),1-\tright(f,\epsilon)]$ denote the bulk of $[0,1]$. We also define $\omega_{\max}(f,x,\epsilon) = \max_{x \in \overline{I}(f,\epsilon)} \omega(f,x\epsilon)$ and $\omega_{\min}(f,\epsilon) = \min_{x \in \overline{I}(f,\epsilon)} \omega(f,x,\epsilon)$. For $t \le \min\{x,1-x\}$, we define the midpoint approximation function $\Delta(f,x,t) = \frac{f(x+t)+f(x-t)}{2} - f(x) = \Delta(f,[x-t,x+t])$. 


Next, by using the sufficient decrease of $\Delta(f,x,t)$, we can express $\Delta(f,x,t)$ as the inverse of $\omega(f,x,\epsilon)$:

	
	Lastly, Lemma~\ref{psi_u_fact} also lets us relate $\omega(f,x,\epsilon)$ and $\omega(f,x,\epsilon')$ as follows.
	
	



	
	

\subsection{Proof of Proposition~\ref{ContinuityProp}}

\begin{lemma}\label{Lem:Positivity} If $f$ is continuous, then for any $\epsilon > 0$, $\tleft(f,\epsilon)$, $\tright(f,\epsilon)$, and $\inf_{x \in [\tleft(f,\epsilon),1-\tright(f,\epsilon)]}\omega(f,x,\epsilon)$ are all strightly postive.
\end{lemma}
\begin{proof}
If $f$ is continuous, then $\lim_{x \to 0} \Delta(f,x,x) \downarrow 0$ and $\lim_{x\to 1} \Delta(f,x,1-x) \downarrow 0$, which implies that $\tleft(f,\epsilon)$ and $\tright(f,\epsilon)$ are positive. Moroever, if $f$ is continuous on $[0,1]$, it is uniformly continuous on $[0,1]$, which implies that there exists a $t$ sufficiently small such that $|f(y)-f(x)| \le \epsilon/2$ whenever $|y-x| \le t$. We may assume without loss of generality that $t \le \min\{\tright(f,\epsilon) ,\tleft(f,\epsilon)\}$, so that $\Delta(f,I)[x-t,x+t]$ is well defined for all $x \in [\tleft(f,\epsilon),1-\tright(f,\epsilon)]$. Then, $\Delta(f,I)[x-t,x+t] \le \frac{1}{2}|f(x+t)-f(x)| + \frac{1}{2}|f(x) - f(x-t)| \le \epsilon/2$. Hence, $\omega(f,x,\epsilon) \ge t$ for all $x \in [\tleft(f,\epsilon),1-\tright(f,\epsilon)]$. 
\end{proof}


\begin{proposition}\label{ContinuityProp} Suppose that $f$ is continuous. Then $\Lambda(f,\epsilon)$ is finite, and $\tleft(f,\epsilon)$, $\tright(f,\epsilon)$, $\Lambda(f,\epsilon)$ and $\underline{N}(f,\epsilon)$ are all right-continuous in $\epsilon$. Moreover, $\omega(f,x,\epsilon)$ is continuous in $\epsilon$.
\end{proposition}

We begin following technical lemma, which relies on the technical preliminaries developed in the previous section.

	\begin{lemma}\label{Lem:RightCont} The maps $\epsilon \mapsto \omega(f,x,\epsilon)$ is continuous for $\epsilon \in [0,\epsilon^*(f,x)]$, and the maps $\epsilon \mapsto \tleft(f,\epsilon)$ and $\epsilon \mapsto \tleft(f,\epsilon)$ are all right-continuous in $\epsilon$. 
	\end{lemma}
	\begin{proof}
	Since $\epsilon \mapsto \omega(f,x,\epsilon)$ on $[0,\epsilon^*(f,x)]$ is given by the inverse of a strictly increasing continuous function, it is continuous on $[0,\epsilon^*(f,x)]$. To see that is right continuous, $\tleft(f,\epsilon)$, take a sequence $\epsilon_i \to \epsilon$. Since $\tleft(f,\epsilon_i)$ is monotone, $t^* = \lim_{i \to \infty} \tleft(f,\epsilon_i)$ exists, and satisfies $t^* \ge \tleft(f,\epsilon)$. Since $\epsilon^*(f,x) = \Delta(f,x,x)$ is continuous in $x$ and satisfies $\epsilon^*(f,\tleft(\epsilon_i)) = \epsilon_i$, we also have $\Delta(f,t^*,t^*) = \epsilon$. Thus, if $t^* \ne t$, then we would have that $t^* > \tleft(f,\epsilon)$ and $\Delta(f,t^*,t^*) = \epsilon$, contradicting the definition of $\tleft(f,\epsilon)$. Right continuity of $\tright$ follows analogously. 
	\end{proof}
	


We can now prove Proposition~\ref{ContinuityProp}:
\begin{proof}
$\Lambda(f,\epsilon)$ is finite since, by Lemma~\ref{Lem:Positivity} $\inf_{x \in [\tleft(f,\epsilon),1-\tright(f,\epsilon)]}\omega(f,x,\epsilon)>0$. To verify right-continuity, Proposition~\ref{LambdaScaleProp} implies that, for any $\lambda \ge 1$,
\begin{eqnarray*}
 \frac{1}{\lambda}\Lambda(f,\epsilon) + \log\frac{\tleft(f,\lambda\epsilon)\tright(f,\lambda\epsilon)}{\tleft(f,\epsilon)\tright(f,\epsilon)} \le \Lambda(f,\epsilon) \le \left\{\Lambda(f,\lambda\epsilon) + \log\frac{\tleft(f,\lambda\epsilon)\tright(f,\lambda\epsilon)}{\tleft(f,\epsilon)\tright(f,\epsilon)} \right\}~.
\end{eqnarray*}
Thus, right-continuity follows as long as $ \log\frac{\tleft(f,\lambda\epsilon)\tright(f,\lambda\epsilon)}{\tleft(f,\epsilon)\tright(f,\epsilon)}$ is right-continuous. By This follows since $\log(\cdot)$ is continuous on $(0,\infty)$, and and $\tleft(f,\epsilon)$ and $\tright(f,\epsilon)$ are right-continuous (Lemma~\ref{Lem:RightCont}) and strictly-positive (Lemma~\ref{Lem:Positivity}). 

To see that $\underline{N}(f,\epsilon)$ is right continuous, we express $\underline{N}(f,\epsilon)$ in terms of $\Lambda(f,\epsilon)$, $\omega_{\max}(f,\epsilon)$, $\omega_{\min}(f,\epsilon)$, the first of which is right-continuous by the above, and the second two of which are right-continuous by Corollary~\ref{cor_min_max_cont} .
\end{proof}


\subsection{Proof of Proposition~\ref{GeneralLambdaScaleProp}}
Finish....


To control $\log(\omega_{\max}(f,\epsilon)/\omega_{\min}(f,\epsilon))$, we use the coarse bound
\begin{eqnarray*}
\log(\omega_{\max}(f,\epsilon)/\omega_{\min}(f,\epsilon)) \le \log(1/\omega_{\min}(f,\epsilon))
\end{eqnarray*}
Thus, by Equation~\eqref{omega_min_max_eq} with $\lambda = 2\|f\|_{\infty}/\epsilon$,
\begin{eqnarray*}
\omega_{\min}(f,\epsilon) &\ge& \frac{\epsilon}{2\|f\|_{\infty}}\min\{\frac{\tleft(f,\epsilon)}{\tleft(f,2\|f\|_{\infty})},\frac{\tright(f,\epsilon)}{\tright(f,2\|f\|_{\infty})} \} \omega_{\min}(f,\infty)\\
&\ge& \frac{\epsilon\tright(f,\epsilon) \tleft(f,\epsilon)}{2\|f\|_{\infty}\tleft(f,\|f\|_{\infty})\tright(f,\|\infty\|)}\omega_{\min}(f,\infty)
\end{eqnarray*}
Finally, since $\|\frac{f(0)+f(1)}{2} - f(1/2)\|_{\infty} \le 2\|f\|_{\infty}$, we have that $\tleft(f,2\|f\|_{\infty}) = \tright(f,2\|\infty\|) = \omega_{\min}(f,2\|f\|_{\infty}) = 1/2$. Hence,
\begin{align*}
\omega_{\min}(f,\epsilon)  \ge \frac{\epsilon\cdot \tright(f,\epsilon) \cdot \tleft(f,\epsilon)}{\|f\|_{\infty}}~.
\end{align*}
Concluding, we find
\begin{align*}
\log(1/\omega_{\min}(f,\epsilon)) \le \log(\|f\|_{\infty}/\epsilon ) + \log(1/\tright(f,\epsilon)) + \log(1/\tleft(f,\epsilon))~.
\end{align*}

\fi
\iffalse
\begin{proof}[Proof of Lemma~\ref{unif_continuity_omega}]
	To prove the first point, let $t = \omega(f,\epsilon,x)$ and $t' = \omega(f,\epsilon',x)$. It is clear from the definition of $\omega$ that $t \ge t'$. Thus, it suffices to show that $t' \ge \frac{\epsilon'}{\epsilon} t$. By the previous part, we have that $\Delta(f,x,t) = \epsilon$ and $\Delta(f,x,t') = \epsilon'$. Thus, by Lemma~\ref{psi_u_fact}, $\epsilon' = \Delta(f,x,t') \le \frac{t'}{t}\Delta(f,x,t) = \frac{t'}{t}\epsilon$. Rearranging, $t' \ge \frac{\epsilon'}{\epsilon} t$. The second point now follows directly from the fact that convex functions $\phi$ satisfying $\phi(0) = 0$ satisfy $\phi(ct) \le c\phi(t)$ for any $c \le 1$ (Lemma~\ref{zero_cvx_lemma})
	\end{proof}


\begin{cor}\label{cor:monotone_lem_cor} Define $\epsilon^*(f,x) := \Delta(f,x,\min\{x,1-x\})$, which represents the error of the midpoint approximation at $x$ on interval $I$ whose endpoints include either $0$ or $1$. $\epsilon^*(f,x)$ is non-decreasing on $[0,1/2]$ and non-increasing on $[1/2,1]$
\end{cor}

\begin{lemma}\label{psi_u_fact}
	Suppose that $f$ is continuous. Then for all $t \in [0,\min\{x,1-x\}]$, the function $\Delta(f,x,t)$ is convex, symmetric, continuous, non-negative and has $\Delta(f,x,0) = 0$. Thus, satisfies $\Delta(f,x,ct)\le c\Delta(f,x,t)$ for all $t \in [0,\min\{x,1-x\}]$ and all $c \le 1$. 
	In particular, if $\Delta(f,x,t') > 0$, then $\Delta(f,x,t)$ is strictly increasing on $t \in [t',\min\{x,1-x\}]$. 
\end{lemma}
\begin{proof}
Writing $\Delta(f,x,t) = \frac{f(x+t)+f(x-t)}{2} + f(x)$, it is immediate that $\Delta(f,x,t)$ is symmetric in $t$. 
Being the sum of affine reparametrizations of a convex, continuous function $f$, $\Delta(f,x,t)$ is convex and continuous. 
By Jensen's inequality, $\frac{f(x+t)+f(x-t)}{2} \ge f(\frac{x+t}{2} + \frac{x-t}{2}) = f(x)$, so $\Delta(f,x,t) \ge 0$.
Since $\Delta(f,x,0) = 0$, convexity implies that $0$ is a global minimimum of $t \mapsto \Delta(f,x,t)$, whence  $\Delta(f,x,t) $ is non-decreasing for $t \ge 0$.
\end{proof}

	\begin{cor}\label{EdgeCor} For any $\lambda \ge 1$ and any $x_1\in [\tleft(f,\epsilon),\tleft(f,\lambda\epsilon)]$ 
	\begin{eqnarray}
	x_1/\lambda \le \omega(f,x_1,\epsilon) \le x_1
	\end{eqnarray}
	Analogous results hold for any $x_2 \in [1-\tright(f,\lambda \epsilon),1-\tright(f,\epsilon)]$. 
	\end{cor}
	\begin{proof}
	Since $x_1 \ge \tleft(f,\epsilon)$, we have $\omega(f,x_1,\epsilon) \le x_1$ by definition. On the other hand, since $x \le \tleft(f,\lambda\epsilon)$, $\epsilon^*(f,x) \le \lambda$. Thus, $\omega(f,x_1,\epsilon)  = \omega(f,x_1,\epsilon^*(f,x) \cdot (\epsilon/\epsilon^*(f,x)) \ge \frac{\epsilon/\epsilon^*(f,x)}  \omega(f,x_1,\epsilon^*(f,x)) \ge \lambda^{-1}\cdot \omega(f,x_1,\epsilon^*(f,x)) =  x_1/\lambda$.
	\end{proof}


Next, we state a result which summarizes Lemma~\ref{unif_continuity_omega} and Corollary~\ref{EdgeCor}: \begin{cor}\label{x_sub_lambda_lem}
	Given $ x \in \overline{I}(f,\epsilon)$ and $\lambda \ge 1$, let 
	\begin{eqnarray}
	x_{\lambda} \in \overline{I}(f,\lambda \epsilon) = \begin{cases} x & x \in  \overline{I}(f,\lambda \epsilon) \\
	\tleft(f,\lambda \epsilon) & x \in  [\tleft(f,\epsilon),\tleft(f,\lambda \epsilon)]\\
	1 - \tright(f,\lambda \epsilon) & x \in [1-\tright(f,\lambda\epsilon),1-\tright(f,\epsilon)] 
	\end{cases} 
	\end{eqnarray}
	Then,
	\begin{eqnarray}
	1 \ge \frac{\omega(f,x,\epsilon)}{\omega(f,x_{\lambda},\lambda\epsilon)}  \ge \begin{cases} 1/\lambda & x \in  \overline{I}(f,\lambda \epsilon) \\
	\frac{\tleft(f,\epsilon)}{\tleft(f,\lambda\epsilon)\lambda}& x \in  [\tleft(f,\epsilon),\tleft(f,\lambda \epsilon)] \\
	\frac{\tright(f,\epsilon)}{\tright(f,\lambda\epsilon)\lambda}& x \in [1-\tright(f,\lambda\epsilon),1-\tright(f,\epsilon)]  
	\end{cases}
	\end{eqnarray}
	\end{cor}

	
	\begin{proof}
	 When $x \in \overline{I}(f,\lambda \epsilon)$, we have by Lemma~\ref{unif_continuity_omega}
	\begin{eqnarray*}
	\frac{1}{\lambda}\omega(f,x,\lambda\epsilon) \le \omega(f,x,\epsilon) \le \omega(f,x,\lambda\epsilon)
	\end{eqnarray*}
	In the second case, Corollary~\ref{EdgeCor} yields that 
	\begin{eqnarray*}
	\lambda^{-1}\tleft(x,f,\epsilon) \le\frac{x}{\lambda} \le  \omega(f,x,\epsilon) \le x \le \tleft(f,\lambda \epsilon)
	\end{eqnarray*}
	The third case follow similarly.
	\end{proof}
	As a direct consequence, we conclude that
	\begin{eqnarray}\label{omega_min_max_eq}
	\frac{1}{\lambda}\min\left\{1,\frac{\tleft(f,\epsilon)}{\tleft(f,\lambda\epsilon)},\frac{\tright(f,\epsilon)}{\tright(f,\lambda\epsilon)}\right\} \le \frac{\omega_{\max}(f,\epsilon)}{\omega_{\max}(f,\lambda \epsilon)},\frac{\omega_{\min}(f,\epsilon)}{\omega_{\min}(f,\lambda \epsilon)} \le 1
	\end{eqnarray}
	so that, by right-continuity of $\tleft(f,\epsilon)$ and $\tright(f,\epsilon)$, we have
	\begin{cor}\label{cor_min_max_cont} $\omega_{\min}(f,\epsilon)$ and $\omega_{\max}(f,\epsilon)$ are right-continuous.
	\end{cor}


Since $f(x+2t)$ and $f(x+t)$ are convex in $t$, they admit right and left derivatives, which we denote by $\partial_{+}$ and $\partial_{-}$. 
Then for $\sigma \in \{+,-\}$, $\frac{\partial_{\sigma}}{\partial_t} f(x+t) = (\partial_{\sigma} f)(x+t)$, and $\frac{\partial_{\sigma}}{\partial_t} (f(x+2t)) = 2 (\partial_{\sigma} f)(x+2t)$. 
Hence, $\Delta(f,x+t,t)$ is both-right and left-differentiable, which $\frac{\partial_{\sigma}}{\partial_t} (\Delta(f,x+t,t)) = (\partial_{\sigma} f)(x+2t) - (\partial_{\sigma} f)(x+t)$. 
Since $f$ is convex, both its right and left derivatives are non-decreasing in $t$. Hence $\frac{\partial_{\sigma}}{\partial_t} (\Delta(f,x+t,t)) \ge 0$, which implies that $\Delta(f,x+t,t)$ is non decreasing.

 Fix $\epsilon \in (0,\epsilon^*(f,x)]$. Since $\epsilon^*(f,x) > 0$, and since $\lim_{t\to 0}\Delta(f,x,t) = 0$ and $\Delta(f,x,t)$ is continuous, there exists some $\epsilon' \in (0,\epsilon)$ and some $t'$ such that $\Delta(f,x,t') = \epsilon'$. Since $\Delta(f,x,t') < \epsilon$ we have that $\omega(f,\epsilon,t) \ge t'$. Hence,
	\begin{eqnarray}
	\omega(f,\epsilon,x) = \sup\{ t \in [t',\min\{x,1-x\}]: \Delta(f,x,t) \le \epsilon\}
	\end{eqnarray}
	Since $\Delta(f,x,t)$ is continuous and strictly increasing on $[t',\min\{u,1-u\}]$, we conclude that $\omega(f,\epsilon,x)$ is the unique $t \in [0,x \wedge (1-x)]$ satisfying $\Delta(f,x,t) = \epsilon$. Moreover, $\Delta(f,x,\omega(f,x,0)) = 0$ follows from the definition of $\Delta$ and continuity of $\omega$.

%That $\epsilon^*(f,x)$ is non-decreasing on $[0,1/2]$ follows by consider $\Delta(f,t,t)$ and that it is non-increasing on $[1/2,1]$ follows by considering $\Delta(f,1-t,t)$.

\fi

